Automatic design of novel potential 3CL$^{\text{pro}}$ and PL$^{\text{pro}}$ inhibitors

With the goal of designing novel inhibitors for SARS-CoV-1 and SARS-CoV-2, we propose the general molecule optimization framework, Molecular Neural Assay Search (MONAS), consisting of three components: a property predictor which identifies molecules with specific desirable properties, an energy model which approximates the statistical similarity of a given molecule to known training molecules, and a molecule search method. In this work, these components are instantiated with graph neural networks (GNNs), Deep Energy Estimator Networks (DEEN) and Monte Carlo tree search (MCTS), respectively. This implementation is used to identify 120K molecules (out of 40-million explored) which the GNN determined to be likely SARS-CoV-1 inhibitors, and, at the same time, are statistically close to the dataset used to train the GNN.

==> Designing Covid Inhibitors (revised)/approach_diagram.tex <==
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw}]
    \node[align=center] (Dataset) at (-6.5, -2) {Dataset of \\SARS-CoV-1 \\inhibition\\ \includegraphics[height=6cm]{mols1.png} \\ \large$\dots$ \\ \vspace{0.1cm}};
    \node[align=center] (GNN) at (-2, 0) {MONAS-P};
    \node[align=center,draw=none,inner sep=0pt] (dpoint) at (-5.4125, 0) {};
    \node[align=center,draw=none,inner sep=0pt] (trn) at (-4.4, 0) {\small Training\\\small data};
    \node[align=center] (DEEN) at (3, 0) {MONAS-E};
    \node[align=center,draw=none,inner sep=0pt] (lat) at (0.5, 0) {\small Feature \\\small space};
    
    \node[align=center] (MCTS) at (0.5, -5) {MONAS-S};
    \node[align=center,draw=none,inner sep=0pt] (prop) at (0.5, -2.5) {\includegraphics[height=1cm]{prop_mol.png}};
    \node[align=center,draw=none,inner sep=0pt] (propdesc) at (-1, -3.75) {\small Proposes \\ \small molecule};
    \node[align=center,draw=none,inner sep=0pt] (propdesc) at (2.5, -3.75) {\small Reward for \\ \small high inhibition, \\ \small high likelihood};
    \node[align=center,draw=none,inner sep=0pt] (mctsrew) at (-2, -1.75) {\small Inhibition \\ \small likelihood};
    \node[align=center,draw=none,inner sep=0pt] (mctsrew) at (3, -1.75) {\small Molecule \\ \small likelihood};
    
    \node[align=center, text width=290, text height = 40] (Out) at (-0.7, -7.25) {};
    \node[align=center,draw=none] (OutDesc) at (-4.7, -7.25) {Dataset of \\proposed novel \\inhibitors};
    \node[align=center,draw=none] (Outpic) at (0, -7.25) {\includegraphics[height=1.25cm]{mols2.png}};
    \node[align=center,draw=none] (Outdot) at (4, -7.25) {\large $\dots$};
    \node[align=center,draw=none,inner sep=0pt] (dpoint2) at (0.5, -6.475) {};
    \node[align=center,draw=none,inner sep=0pt] (outde) at (0.5, -5.75) {\small Best discovered molecules};
\end{scope}

\begin{scope}[every node/.style={fill=white,circle},
              every edge/.style={draw=black,thick}]
            
            
            \path [] (dpoint) edge (trn);
            \path [->] (trn) edge (GNN);
            
            \path [] (GNN) edge (lat);
            \path [->] (lat) edge (DEEN);
            
            
            \path [->,out=135,in=235] (MCTS) edge (prop);
            \path [->,out=305,in=45] (prop) edge (MCTS);
            
            \path [->,out=300,in=160,looseness=1] (GNN) edge (prop);
            \path [->,out=120,in=330] (prop) edge (GNN);
            
            \path [->,out=240,in=20,looseness=1] (DEEN) edge (prop);
            \path [->,out=60,in=210] (prop) edge (DEEN);
            
            
            
            \path [] (MCTS) edge (outde);
            \path [->] (outde) edge (dpoint2);
\end{scope}
\end{tikzpicture}

% \begin{tikzpicture}
% \begin{scope}[every node/.style={rectangle,thick,draw}]
%     \node[align=center] (Dataset) at (-6.5, -2) {Dataset of \\SARS-CoV-1 \\inhibition\\ \includegraphics[height=6cm]{mols1.png} \\ \large$\dots$ \\ \vspace{0.1cm}};
%     \node[align=center] (GNN) at (-2, 0) {Inhibition \\ predictor};
%     \node[align=center,draw=none,inner sep=0pt] (dpoint) at (-5.4125, 0) {};
%     \node[align=center,draw=none,inner sep=0pt] (trn) at (-4.4, 0) {\small Training\\\small data};
%     \node[align=center] (DEEN) at (3, 0) {Energy \\model };
%     \node[align=center,draw=none,inner sep=0pt] (lat) at (0.5, 0) {\small Feature \\\small space};
    
%     \node[align=center] (MCTS) at (0.5, -5) {Directed search};
%     \node[align=center,draw=none,inner sep=0pt] (prop) at (0.5, -2.5) {\includegraphics[height=1cm]{prop_mol.png}};
%     \node[align=center,draw=none,inner sep=0pt] (propdesc) at (-1, -3.75) {\small Proposes \\ \small molecule};
%     \node[align=center,draw=none,inner sep=0pt] (propdesc) at (2.5, -3.75) {\small Reward for \\ \small high inhibition, \\ \small high likelihood};
%     \node[align=center,draw=none,inner sep=0pt] (mctsrew) at (-2, -1.75) {\small Inhibition \\ \small likelihood};
%     \node[align=center,draw=none,inner sep=0pt] (mctsrew) at (3, -1.75) {\small Molecule \\ \small likelihood};
    
%     \node[align=center, text width=290, text height = 40] (Out) at (-0.7, -7.25) {};
%     \node[align=center,draw=none] (OutDesc) at (-4.7, -7.25) {Dataset of \\proposed novel \\inhibitors};
%     \node[align=center,draw=none] (Outpic) at (0, -7.25) {\includegraphics[height=1.25cm]{mols2.png}};
%     \node[align=center,draw=none] (Outdot) at (4, -7.25) {\large $\dots$};
%     \node[align=center,draw=none,inner sep=0pt] (dpoint2) at (0.5, -6.475) {};
%     \node[align=center,draw=none,inner sep=0pt] (outde) at (0.5, -5.75) {\small Best discovered molecules};
% \end{scope}

% \begin{scope}[every node/.style={fill=white,circle},
%               every edge/.style={draw=black,thick}]
            
            
%             \path [] (dpoint) edge (trn);
%             \path [->] (trn) edge (GNN);
            
%             \path [] (GNN) edge (lat);
%             \path [->] (lat) edge (DEEN);
            
            
%             \path [->,out=135,in=235] (MCTS) edge (prop);
%             \path [->,out=305,in=45] (prop) edge (MCTS);
            
%             \path [->,out=300,in=160,looseness=1] (GNN) edge (prop);
%             \path [->,out=120,in=330] (prop) edge (GNN);
            
%             \path [->,out=240,in=20,looseness=1] (DEEN) edge (prop);
%             \path [->,out=60,in=210] (prop) edge (DEEN);
            
            
            
%             \path [] (MCTS) edge (outde);
%             \path [->] (outde) edge (dpoint2);
% \end{scope}
% \end{tikzpicture}

==> Designing Covid Inhibitors (revised)/mcts.tex <==

\textbf{1. Selection}\\
\begin{center}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
\end{scope}
\end{tikzpicture}\\
\end{center}
\vspace{0.2cm}

\textbf{2. Expansion}\\
\begin{center}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center] (V10) at (-4, -1) {{\small\textbf{V1}}};
    \node[align=center,draw=blue] (V11) at (0, -1) {{\small\textbf{V2};\textbf{SB}}};
    \node[align=center] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->] (V00) edge  (V10);
            \path [->] (V00) edge[draw=blue,blue]  (V11);
            \path [->] (V00) edge  (V12);
\end{scope}
\end{tikzpicture}\\
\end{center}
\vspace{0.2cm}

\textbf{3. Rollout}\\
\begin{center}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center, draw = gray] (V10) at (-4, -1) {{\small\textbf{V1}}};
    \node[align=center, draw = blue] (V11) at (0, -1) {{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=gray] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    \node[align=center, draw=none,text width = 2.5cm] (Mol) at (0, -2.6) {\includegraphics[width=2cm]{prop_mol.png}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->, dashed] (V00) edge[gray, draw=gray, fill=gray]  (V10);
            \path [->] (V00) edge[draw=blue,blue]  (V11);
            \path [->, dashed] (V00) edge[gray, draw=gray, fill=gray]  (V12);
            \path [->,snake=zigzag] (V11) edge[snake]  (Mol);
\end{scope}
\end{tikzpicture}\\
\end{center}
\vspace{0.2cm}

\textbf{4. Backpropagation}\\
\begin{center}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center, draw = gray] (V10) at (-4, -1) {{\small\textbf{V1}}};
    \node[align=center, draw = blue] (V11) at (0, -1) {{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=gray] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    \node[align=center, draw=none,text width = 2.5cm] (Mol) at (0, -2.6) {\includegraphics[width=2cm]{prop_mol.png}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->, dashed] (V00) edge[gray, draw=gray, fill=gray]  (V10);
            \path [->] (V00) edge[draw=blue,blue]  (V11);
            \path [->, dashed] (V00) edge[gray, draw=gray, fill=gray]  (V12);
            \path [->,snake=zigzag] (V11) edge[snake]  (Mol);
            
            \path [->,out=0,in=350] (Mol) edge[draw=green!50!black] node{$w_\beta(G)$} (V11);
            \path [->,out=10,in=360, looseness = 3] (V11) edge[draw=green!50!black] node{$w_\beta(G)$} (V00);
\end{scope}
\end{tikzpicture}\\
\end{center}

\begin{center}
    - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\end{center}
\vspace{0.2cm}

\textbf{1. Selection}\\
\begin{center}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center] (V10) at (-4, -1) {{\small\textbf{V1}}};
    \node[align=center] (V11) at (0, -1) {{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->] (V00) edge  (V10);
            \path [->] (V00) edge  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
\end{scope}
\end{tikzpicture}\\
\end{center}

\textbf{2. Expansion}\\
\begin{center}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center] (V10) at (-4, -1) {{\small\textbf{V1}}};
    \node[align=center] (V11) at (0, -1) {{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=blue] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\large $\dots$};
    \node[align=center,text width=1.75cm] (V25) at (7, -2) {\small [C@H];\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\large $\dots$};
    \node[align=center,draw=none,text width=1.75cm] (NULL) at (-7, -2) {\small };
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->, dashed] (V00) edge[fill=gray,gray]  (V10);
            \path [->, dashed] (V00) edge[fill=gray,gray] (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->,draw=blue,blue] (V12) edge[draw=blue,blue]  (V24);
            \path [->] (V12) edge  (V2dot2);
            \path [->] (V12) edge  (V25);
\end{scope}
\end{tikzpicture}\\
\end{center}

==> Designing Covid Inhibitors (revised)/mcts_old.tex <==
\centering
\textbf{1. Selection}\\\vspace{0.4cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center] (V10) at (-4, -1) {\small\textbf{V1}};
    \node[align=center] (V11) at (0, -1) {\small\textbf{V2};\textbf{SB}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\small F};
    \node[align=center,draw=none] (V2dot1) at (-5, -2) {\large $\dots$};
    \node[align=center,draw=none] (V21) at (-4, -2) {\small Cl};
    
    \node[align=center] (V22) at (-1.5, -2) {\small O; \textbf{SB}};
    \node[align=center] (V23) at (1.5, -2) {\small S; \textbf{SB}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\large $\dots$};
    \node[align=center,text width=1.75cm] (V25) at (7, -2) {\small [C@H];\textbf{DB}};
    
    
    \node[align=center,draw=none] (V3dot1) at (-1.5, -3) {\large $\dots$};
    \node[align=center,draw=none] (V3dot2) at (1.5, -3) {\large $\dots$};
    \node[align=center,draw=none] (V3dot3) at (7, -3) {\large $\dots$};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->] (V00) edge  (V10);
            \path [->] (V00) edge  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V10) edge  (V20);
            \path [->] (V10) edge  (V2dot1);
            \path [->] (V10) edge  (V21);
            
            \path [->] (V11) edge  (V22);
            \path [->] (V11) edge  (V23);
            
            \path [->,draw=red,red] (V12) edge[draw=red,red]  (V24);
            \path [->] (V12) edge  (V2dot2);
            \path [->] (V12) edge  (V25);
            
            
            \path [->] (V22) edge  (V3dot1);
            \path [->] (V23) edge  (V3dot2);
            \path [->] (V25) edge  (V3dot3);
\end{scope}
\end{tikzpicture}\\\vspace{0.4cm}

\textbf{2. Expansion}\\\vspace{0.2cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center,draw=gray] (V10) at (-4, -1) {\textcolor{gray}{\small\textbf{V1}}};
    \node[align=center,draw=gray] (V11) at (0, -1) {\textcolor{gray}{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\textcolor{white}{\small F}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\textcolor{gray}{\large $\dots$}};
    \node[align=center,text width=1.75cm,draw=gray] (V25) at (7, -2) {\textcolor{gray}{\small [C@H];\textbf{DB}}};
    
    
    \node[align=center] (V31) at (1.5, -3) {\small N=;\textbf{V2}};
    \node[align=center, text width=1.75cm,draw=blue] (V32) at (4, -3) {\small N=;\textbf{V3};\textbf{NH}};
    \node[align=center,draw=none] (V33) at (5.5, -3) {\large $\dots$};
    \node[align=center, text width=1.75cm] (V34) at (7, -3) {\small N=;\textbf{V4};\textbf{DB}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V10);
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V12) edge[draw=red,red]  (V24);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V2dot2);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V25);
            
            \path [->] (V24) edge  (V31);
            \path [->] (V24) edge[draw=blue,blue]  (V32);
            \path [->] (V24) edge  (V34);
\end{scope}
\end{tikzpicture}\\\vspace{0.4cm}

\textbf{3. Rollout}\\\vspace{0.2cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center,draw=gray] (V10) at (-4, -1) {\textcolor{gray}{\small\textbf{V1}}};
    \node[align=center,draw=gray] (V11) at (0, -1) {\textcolor{gray}{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\textcolor{white}{\small F}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\textcolor{gray}{\large $\dots$}};
    \node[align=center,text width=1.75cm,draw=gray] (V25) at (7, -2) {\textcolor{gray}{\small [C@H];\textbf{DB}}};
    
    
    \node[align=center,draw=gray] (V31) at (1.5, -3) {\textcolor{gray}{\small N=;\textbf{V2}}};
    \node[align=center, text width=1.75cm,draw=blue] (V32) at (4, -3) {\small N=;\textbf{V3};\textbf{NH}};
    \node[align=center,draw=none] (V33) at (5.5, -3) {\large $\dots$};
    \node[align=center, text width=1.75cm,draw=gray] (V34) at (7, -3) {\textcolor{gray}{\small N=;\textbf{V4};\textbf{DB}}};
    
    \node[align=center, draw=none] (G) at (2.75, -4.6) {$G$:};
    \node[align=center, draw=none,text width = 2.5cm] (Mol) at (4, -4.6) {\includegraphics[width=2cm]{prop_mol.png}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V10);
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V12) edge[draw=red,red]  (V24);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V2dot2);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V25);
            
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V31);
            \path [->] (V24) edge[draw=blue,blue]  (V32);
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V34);
            \path [->,snake=zigzag] (V32) edge[snake]  (Mol);
\end{scope}
\end{tikzpicture}\\\vspace{0.2cm}

\textbf{4. Backpropagation}\\\vspace{0.2cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center,draw=gray] (V10) at (-4, -1) {\textcolor{gray}{\small\textbf{V1}}};
    \node[align=center,draw=gray] (V11) at (0, -1) {\textcolor{gray}{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\textcolor{white}{\small F}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\textcolor{gray}{\large $\dots$}};
    \node[align=center,text width=1.75cm,draw=gray] (V25) at (7, -2) {\textcolor{gray}{\small [C@H];\textbf{DB}}};
    
    
    \node[align=center,draw=gray] (V31) at (1.5, -3) {\textcolor{gray}{\small N=;\textbf{V2}}};
    \node[align=center, text width=1.75cm,draw=blue] (V32) at (4, -3) {\small N=;\textbf{V3};\textbf{NH}};
    \node[align=center,draw=none] (V33) at (5.5, -3) {\large $\dots$};
    \node[align=center, text width=1.75cm,draw=gray] (V34) at (7, -3) {\textcolor{gray}{\small N=;\textbf{V4};\textbf{DB}}};
    
    \node[align=center, draw=none] (G) at (2.75, -4.6) {$G$:};
    \node[align=center, draw=none,text width = 2.5cm] (Mol) at (4, -4.6) {\includegraphics[width=2cm]{prop_mol.png}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V10);
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V12) edge[draw=red,red]  (V24);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V2dot2);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V25);
            
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V31);
            \path [->] (V24) edge[draw=blue,blue]  (V32);
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V34);
            \path [->,snake=zigzag] (V32) edge[snake]  (Mol);
            
            
            \path [->,out=0,in=350] (Mol) edge[draw=green!50!black] node{$w_\beta(G)$} (V32);
            \path [->,out=0,in=0,looseness=3] (V32) edge[draw=green!50!black] node{$w_\beta(G)$} (V24);
            \path [->,out=0,in=0,looseness=3] (V24) edge[draw=green!50!black] node{$w_\beta(G)$} (V12);
            \path [->,out=90,in=0] (V12) edge[draw=green!50!black] node{$w_\beta(G)$} (V00);
\end{scope}
\end{tikzpicture}\\

==> Designing Covid Inhibitors (revised)/model.tex <==
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw}]
    \node[align=center,draw=none] (X) at (3, -0.5) {$G$};
    \coordinate (GEC1con) at (3, -1.25);
    \node[align=center] (GEC1) at (3, -2) {GEC\textsubscript{1}};
    \coordinate (GEC2con) at (3, -3);
    \node[align=center] (GEC2) at (3, -4) {GEC\textsubscript{2}};
    \coordinate (GEC3con) at (3, -5);
    \node[align=center] (GEC3) at (3, -6) {GEC\textsubscript{3}};
    \coordinate (GEC4con) at (3, -7);
    
    %Connector down LHS
    
    \coordinate (GEC1L) at (0, -3);
    
    \draw (0,-5) circle (6pt);
    \coordinate (GEC2Lcon) at (0, -4);
    \node[cross=5pt,rotate=45,black] (GEC2L) at (0, -5) {};
    
    \draw (0,-7) circle (6pt);
    \coordinate (GEC3Lcon) at (0, -6);
    \node[cross=5pt,rotate=45,black] (GEC3L) at (0, -7) {};
    
    \coordinate (GEC4Lcon) at (0, -8);
    \coordinate (headcon) at (0,-9.5);
    
    \coordinate (deenarr) at (0,-10.75);
    \node[align=center] (deen) at (0,-12) {DEEN};
    
    
    %Circle
    \coordinate (csrc1) at (3.6, -2);
    \coordinate (ctrg1) at (8.5, -1.9);
    \coordinate (ctrg2) at (5.7, -5.5);
    \path [dashed] (csrc1) edge (ctrg1);
    \path [dashed] (csrc1) edge (ctrg2);
    \draw[fill=white] (8.4, -4.75) circle (82pt);
    
    %MLPS
    \coordinate (poolarr) at (0.75, -9.5);
    
    \coordinate (poolsplit) at (1.5, -9.5);
    \coordinate (poolsplittop) at (1.5, -8);
    \coordinate (poolsplittop2) at (1.5, -9);
    \coordinate (poolsplitbot2) at (1.5, -10);
    \coordinate (poolsplitbot) at (1.5, -11);
    
    \node[align=center,minimum width = 4cm] (MLP1) at (4.5, -8) {MLP for Assay 1,706};
    \node[align=center,minimum width = 4cm] (MLP2) at (4.5, -9) {MLP for Assay 1,879};
    \node[align=center,minimum width = 4cm] (MLP3) at (4.5, -10) {MLP for Assay 485,353};
    \node[align=center,minimum width = 4cm] (MLP4) at (4.5, -11) {MLP for Assay 652,038};
    
    \coordinate (poolmergetop) at (7.5, -8);
    \coordinate (poolmergetop2) at (7.5, -9);
    \coordinate (poolmergebot2) at (7.5, -10);
    \coordinate (poolmergebot) at (7.5, -11);
    
    
    \draw (7.5,-9.5) circle (6pt);
    
    \node[cross=5pt,rotate=45,black] (poolmerge) at (7.5, -9.5) {};
    \coordinate (presig) at (8.25, -9.5);
    \coordinate (postsig) at (9.75, -9.5);
    
    \node[align=center,draw=none] (MX) at (10.75, -9.5) {$f(G)$};
    \node[align=center,draw=none] (EX) at (10.75, -12) {$\e(X)$};
    
    %GN layer
    \node[align=center,draw=none] (V) at (7, -3) {$V_k$};
    \coordinate (Vcon) at (7, -3.5);
    \node[align=center,draw=none] (E) at (10, -3) {$E_k$};
    \coordinate (Econ) at (10, -3.5);
    \node[align=center, minimum height=0.6cm] (EMLP) at (10, -4) {\small Edge MLP};
    \node[align=center, minimum height=0.6cm] (VMLP) at (7, -4) {\small Node MLP};
    \coordinate (VEcon) at (8.5, -4);
    \coordinate (VTopKcon) at (7, -4.75);
    \coordinate (ETopKcon) at (10, -4.75);
    \coordinate (ETopKcon2) at (10, -5.5);
    \node[align=center, minimum height=0.6cm] (TopK) at (7, -5.5) {\small Edge Pooling};
    
    \node[align=center,draw=none] (Vpr) at (7, -6.5) {$V_{k+1}$};
    \coordinate (Vprcon) at (7, -6);
    \node[align=center,draw=none] (Epr) at (10, -6.5) {$E_{k+1}$};
    \coordinate (Eprcon) at (10, -6);
    
\end{scope}

\begin{scope}[every node/.style={fill=white,circle},
              every edge/.style={draw=black,thick}]
            \path [->] (X) edge (GEC1con);
            \path [] (GEC1con) edge (GEC1);
            \path [->] (GEC1) edge (GEC2con);
            \path [] (GEC2con) edge (GEC2);
            \path [->] (GEC2) edge (GEC3con);
            \path [] (GEC3con) edge (GEC3);
            \path [] (GEC3) edge (GEC4con);
            
            \path [] (GEC2con) edge node {\small Mean/Max} (GEC1L);
            \path [] (GEC3con) edge node {\small Mean/Max} (GEC2L);
            \path [] (GEC4con) edge node {\small Mean/Max} (GEC3L);
              
            \path [->] (GEC1L) edge (GEC2Lcon);
            \path [] (GEC2Lcon) edge (GEC2L);
              
            \path [->] (GEC2L) edge (GEC3Lcon);
            \path [] (GEC3Lcon) edge (GEC3L);
            
            \path [->] (GEC3L) edge (GEC4Lcon);
            \path [] (GEC4Lcon) edge (headcon);
            
            \path [->] (headcon) edge (poolarr);
            \path [] (poolarr) edge (poolsplit);
            \path [] (poolsplittop) edge (poolsplitbot);
            
            \path [] (poolsplittop) edge (MLP1);
            \path [] (poolsplittop2) edge (MLP2);
            \path [] (poolsplitbot2) edge (MLP3);
            \path [] (poolsplitbot) edge (MLP4);
            
            \path [] (MLP1) edge (poolmergetop);
            \path [] (MLP2) edge (poolmergetop2);
            \path [] (MLP3) edge (poolmergebot2);
            \path [] (MLP4) edge (poolmergebot);
            
            \path [] (poolmergetop) edge (poolmerge);
            \path [] (poolmergebot) edge (poolmerge);
            
            \path [->] (poolmerge) edge (presig);
            \path [] (presig) edge node {\small Sigmoid} (postsig);
            \path [->] (postsig) edge (MX);
            
            \path [->] (headcon) edge node {$\X$} (deenarr);
            \path [] (deenarr) edge (deen);
            \path [->] (deen) edge (EX);
            
            %Connections for zoom in on GEC
            
            \path [->] (V) edge (Vcon);
            \path [] (Vcon) edge (VMLP);
            \path [->] (E) edge (Econ);
            \path [] (Econ) edge (EMLP);
            \path [->] (EMLP) edge (VEcon);
            \path [] (VEcon) edge (VMLP);
            
            \path [->] (VMLP) edge (VTopKcon);
            \path [] (VTopKcon) edge (TopK);
            
            \path [->] (EMLP) edge (ETopKcon);
            \path [] (ETopKcon) edge (ETopKcon2);
            \path [] (ETopKcon2) edge (TopK);
            
            \path [] (TopK) edge (Vprcon);
            \path [->] (Vprcon) edge (Vpr);
            \path [] (Vprcon) edge (Eprcon);
            \path [->] (Eprcon) edge (Epr);
\end{scope}
\end{tikzpicture}

==> mcts_old.tex <==
\centering
\textbf{1. Selection}\\\vspace{0.4cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center] (V10) at (-4, -1) {\small\textbf{V1}};
    \node[align=center] (V11) at (0, -1) {\small\textbf{V2};\textbf{SB}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\small F};
    \node[align=center,draw=none] (V2dot1) at (-5, -2) {\large $\dots$};
    \node[align=center,draw=none] (V21) at (-4, -2) {\small Cl};
    
    \node[align=center] (V22) at (-1.5, -2) {\small O; \textbf{SB}};
    \node[align=center] (V23) at (1.5, -2) {\small S; \textbf{SB}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\large $\dots$};
    \node[align=center,text width=1.75cm] (V25) at (7, -2) {\small [C@H];\textbf{DB}};
    
    
    \node[align=center,draw=none] (V3dot1) at (-1.5, -3) {\large $\dots$};
    \node[align=center,draw=none] (V3dot2) at (1.5, -3) {\large $\dots$};
    \node[align=center,draw=none] (V3dot3) at (7, -3) {\large $\dots$};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->] (V00) edge  (V10);
            \path [->] (V00) edge  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V10) edge  (V20);
            \path [->] (V10) edge  (V2dot1);
            \path [->] (V10) edge  (V21);
            
            \path [->] (V11) edge  (V22);
            \path [->] (V11) edge  (V23);
            
            \path [->,draw=red,red] (V12) edge[draw=red,red]  (V24);
            \path [->] (V12) edge  (V2dot2);
            \path [->] (V12) edge  (V25);
            
            
            \path [->] (V22) edge  (V3dot1);
            \path [->] (V23) edge  (V3dot2);
            \path [->] (V25) edge  (V3dot3);
\end{scope}
\end{tikzpicture}\\\vspace{0.4cm}

\textbf{2. Expansion}\\\vspace{0.2cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center,draw=gray] (V10) at (-4, -1) {\textcolor{gray}{\small\textbf{V1}}};
    \node[align=center,draw=gray] (V11) at (0, -1) {\textcolor{gray}{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\textcolor{white}{\small F}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\textcolor{gray}{\large $\dots$}};
    \node[align=center,text width=1.75cm,draw=gray] (V25) at (7, -2) {\textcolor{gray}{\small [C@H];\textbf{DB}}};
    
    
    \node[align=center] (V31) at (1.5, -3) {\small N=;\textbf{V2}};
    \node[align=center, text width=1.75cm,draw=blue] (V32) at (4, -3) {\small N=;\textbf{V3};\textbf{NH}};
    \node[align=center,draw=none] (V33) at (5.5, -3) {\large $\dots$};
    \node[align=center, text width=1.75cm] (V34) at (7, -3) {\small N=;\textbf{V4};\textbf{DB}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V10);
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V12) edge[draw=red,red]  (V24);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V2dot2);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V25);
            
            \path [->] (V24) edge  (V31);
            \path [->] (V24) edge[draw=blue,blue]  (V32);
            \path [->] (V24) edge  (V34);
\end{scope}
\end{tikzpicture}\\\vspace{0.4cm}

\textbf{3. Rollout}\\\vspace{0.2cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center,draw=gray] (V10) at (-4, -1) {\textcolor{gray}{\small\textbf{V1}}};
    \node[align=center,draw=gray] (V11) at (0, -1) {\textcolor{gray}{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\textcolor{white}{\small F}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\textcolor{gray}{\large $\dots$}};
    \node[align=center,text width=1.75cm,draw=gray] (V25) at (7, -2) {\textcolor{gray}{\small [C@H];\textbf{DB}}};
    
    
    \node[align=center,draw=gray] (V31) at (1.5, -3) {\textcolor{gray}{\small N=;\textbf{V2}}};
    \node[align=center, text width=1.75cm,draw=blue] (V32) at (4, -3) {\small N=;\textbf{V3};\textbf{NH}};
    \node[align=center,draw=none] (V33) at (5.5, -3) {\large $\dots$};
    \node[align=center, text width=1.75cm,draw=gray] (V34) at (7, -3) {\textcolor{gray}{\small N=;\textbf{V4};\textbf{DB}}};
    
    \node[align=center, draw=none] (G) at (2.75, -4.6) {$G$:};
    \node[align=center, draw=none,text width = 2.5cm] (Mol) at (4, -4.6) {\includegraphics[width=2cm]{prop_mol.png}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V10);
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V12) edge[draw=red,red]  (V24);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V2dot2);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V25);
            
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V31);
            \path [->] (V24) edge[draw=blue,blue]  (V32);
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V34);
            \path [->,snake=zigzag] (V32) edge[snake]  (Mol);
\end{scope}
\end{tikzpicture}\\\vspace{0.2cm}

\textbf{4. Backpropagation}\\\vspace{0.2cm}
\begin{tikzpicture}
\begin{scope}[every node/.style={rectangle,thick,draw,minimum size=0.6cm, text width=1.25cm}]
    \node[align=center,draw=red] (V00) at (0, 0) {\small\textbf{S}};
    \node[align=center,draw=gray] (V10) at (-4, -1) {\textcolor{gray}{\small\textbf{V1}}};
    \node[align=center,draw=gray] (V11) at (0, -1) {\textcolor{gray}{\small\textbf{V2};\textbf{SB}}};
    \node[align=center,draw=red] (V12) at (4, -1) {\small\textbf{V3};\textbf{DB}};
    
    \node[align=center,draw=none] (V20) at (-6, -2) {\textcolor{white}{\small F}};
    
    \node[align=center,draw=red] (V24) at (4, -2) {\small N;\textbf{DB}};
    \node[align=center,draw=none] (V2dot2) at (5.5, -2) {\textcolor{gray}{\large $\dots$}};
    \node[align=center,text width=1.75cm,draw=gray] (V25) at (7, -2) {\textcolor{gray}{\small [C@H];\textbf{DB}}};
    
    
    \node[align=center,draw=gray] (V31) at (1.5, -3) {\textcolor{gray}{\small N=;\textbf{V2}}};
    \node[align=center, text width=1.75cm,draw=blue] (V32) at (4, -3) {\small N=;\textbf{V3};\textbf{NH}};
    \node[align=center,draw=none] (V33) at (5.5, -3) {\large $\dots$};
    \node[align=center, text width=1.75cm,draw=gray] (V34) at (7, -3) {\textcolor{gray}{\small N=;\textbf{V4};\textbf{DB}}};
    
    \node[align=center, draw=none] (G) at (2.75, -4.6) {$G$:};
    \node[align=center, draw=none,text width = 2.5cm] (Mol) at (4, -4.6) {\includegraphics[width=2cm]{prop_mol.png}};
\end{scope}

\begin{scope}[every node/.style={fill=white,rectangle,draw=none, inner sep =2pt},
              every edge/.style={draw=black,thick}]
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V10);
            \path [->,dashed] (V00) edge[gray,draw=gray,fill=gray]  (V11);
            \path [->] (V00) edge[draw=red,red]  (V12);
            
            \path [->] (V12) edge[draw=red,red]  (V24);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V2dot2);
            \path [->,dashed] (V12) edge[gray,draw=gray,fill=gray]  (V25);
            
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V31);
            \path [->] (V24) edge[draw=blue,blue]  (V32);
            \path [->,dashed] (V24) edge[gray,draw=gray,fill=gray]  (V34);
            \path [->,snake=zigzag] (V32) edge[snake]  (Mol);
            
            
            \path [->,out=0,in=350] (Mol) edge[draw=green!50!black] node{$w_\beta(G)$} (V32);
            \path [->,out=0,in=0,looseness=3] (V32) edge[draw=green!50!black] node{$w_\beta(G)$} (V24);
            \path [->,out=0,in=0,looseness=3] (V24) edge[draw=green!50!black] node{$w_\beta(G)$} (V12);
            \path [->,out=90,in=0] (V12) edge[draw=green!50!black] node{$w_\beta(G)$} (V00);
\end{scope}
\end{tikzpicture}\\
